Spectral variability of the IR-source IRAS 01005+7910 optical component

Highly-resolution optical spectra of the optical component of the IR-source IRAS01005+7910 are used to determine the spectral type of its central star, B1.5$ \pm $0.3, identify the spectral features, and analyze their profile and radial velocity variations. The systemic velocity Vsys =$-50.5$ km/s is determined from the positions of the symmetric and stable profiles of the forbidden [NI], [NII], [OI], [SII], and [FeII] emission lines. The presence of the [NII] and [SII] forbidden emissions indicates the onset of the ionization of the circumstellar envelope and the fact that the star is very close to undergoing the planetary nebula stage. The broad range of heliocentric radial velocity Vr estimates based on the core lines, which amounts to about 34 km/s, is partly due to the deformations of the profiles caused by variable emissions. The variations of the Vr in the line wings are smaller, about 23 km/s, and may be due to pulsations and/or hidden binarity of the star. The deformations of the profiles of complex absorption-emission lines may result from variations of their absorption components caused by the variations of the geometry and kinematics in the wind base. The H$\alpha$ lines exhibit P Cyg III type wind profiles. Deviations of the wind from spherical symmetry are shown to be small. The relatively low wind velocity (27$\div$74 km/s from different observations) and the strong intensity of the red emission (it exceeds the continuum level by up to a factor of seven) are typical for hypergiants rather than the classical supergiants. IRAS01005 +7910 is an example of spectral mimicry of a low mass post-AGB star masquerading as a massive hypergiant.

==> longtab.tex <==

\begin{longtable}{l llc@{\quad} @{\quad}l @{\quad}l @{\quad}l@{\quad}}
\caption{Отождествление линий, их остаточные интенсивности
              и лучевые скорости ${\rm V_r }$\,, км/сек в спектре
	      Cyg\,OB2 - ${\rm \No}$\,12. В скобках указан номер мультиплета
	      }      
\\ \hline
\endfirsthead
\hline
\multicolumn{6}{l}{Табл.\,1, продолжение} \\ \hline
\endhead
\hline
\multicolumn{6}{r}{продолжение на след. странице} \\ \hline
\endfoot
\hline
\endlastfoot
\hline
 Е & & ${\rm \lambda_{lab}}$ &  W$_{\lambda}$, \AA & r  & ${\rm V_r }$  \\
\hline

\hline
\end{longtable}	       			     
\label{lines}

